Observation and Polarization Measurement of B0 --> a1(1260)+ a1(1260)- Decay

We present measurements of the branching fraction B and the longitudinal polarization fraction fL for B0 -> a1(1260)+ a1(1260)- decays, with a1(1260)+/- -> \pi- \pi+ \pi+/-. The data sample, collected with the detector BaBar at the SLAC National Accelerator Laboratory, represents 465 10^6 produced BBbar pairs. We measure B(B0 -> a1(1260)+ a1(1260)-) x [B(a1(1260)+ -> \pi- \pi+ \pi+)]^2 = (11.8 \pm 2.6 \pm 1.6) 10^{-6} and fL = 0.31 \pm 0.22 \pm 0.10, where the first uncertainty is statistical and the second systematic. The decay mode is measured with a significance of 5.0 standard deviations including systematic uncertainties.

==> abstract.tex <==
We present measurements of the branching fraction \mbox{${\cal B}$}\ and 
longitudinal polarization fraction \mbox{$f_L$}\ for
\mbox{$B^0 \rightarrow  a_1(1260)^+  a_1(1260)^- $}\
decays, with $a_1(1260)^{\pm} \rightarrow  \pi^- \pi^+ \pi^{\pm} $.
The data sample, collected with the  detector {{\em B}{\footnotesize\em A}{\em B}{\footnotesize\em AR}}\
at the SLAC National Accelerator Laboratory, represents $465 \times 10^6$\ produced
{\ensuremath{B\overline{B}{}}}\ pairs.
We measure  ${\mbox{$\cal B(\mbox{$B^0 \rightarrow \mbox{$a_1(1260)^+  $}
\mbox{$a_1(1260)^-  $} $} )$}} \times [\mbox{${  \cal    B}$} {\mbox{$({\mbox{$a_1(1260)^+ 
\rightarrow  \pi^- \pi^+ \pi^+ $}} )$}]^2 = \ensuremath{{(11.8 \pm 2.6 \pm 1.6)}}\times 10^{-6}}$\
and $\mbox{$f_L$}\  = 0.31 \pm 0.22 \pm 0.10$, where the first uncertainty is statistical
and the second systematic.
The decay mode is measured with a significance of 5.0
standard deviations including systematic uncertainties.
